Multi-Attention Multi-Class Constraint for Fine-grained Image Recognition

Attention-based learning for fine-grained image recognition remains a challenging task, where most of the existing methods treat each object part in isolation, while neglecting the correlations among them. In addition, the multi-stage or multi-scale mechanisms involved make the existing methods less efficient and hard to be trained end-to-end. In this paper, we propose a novel attention-based convolutional neural network (CNN) which regulates multiple object parts among different input images. Our method first learns multiple attention region features of each input image through the one-squeeze multi-excitation (OSME) module, and then apply the multi-attention multi-class constraint (MAMC) in a metric learning framework. For each anchor feature, the MAMC functions by pulling same-attention same-class features closer, while pushing different-attention or different-class features away. Our method can be easily trained end-to-end, and is highly efficient which requires only one training stage. Moreover, we introduce Dogs-in-the-Wild, a comprehensive dog species dataset that surpasses similar existing datasets by category coverage, data volume and annotation quality. This dataset will be released upon acceptance to facilitate the research of fine-grained image recognition. Extensive experiments are conducted to show the substantial improvements of our method on four benchmark datasets.

==> useful.tex <==
%\documentclass[10pt]{llncs}
\usepackage[usenames]{color} %used for font color
\usepackage{amssymb} %maths
\usepackage{amsmath} %maths
\usepackage[utf8]{inputenc} %useful to type directly diacritic characters
\begin{document}
\[% Bold Captial Symbols
\newcommand{\A}{\mathbf{A}}
\newcommand{\B}{\mathbf{B}}
\newcommand{\C}{\mathbf{C}}
\newcommand{\D}{\mathbf{D}}
\newcommand{\E}{\mathbf{E}}
\newcommand{\F}{\mathbf{F}}
\newcommand{\G}{\mathbf{G}}
\newcommand{\bH}{\mathbf{H}}
\newcommand{\I}{\mathbf{I}}
\newcommand{\J}{\mathbf{J}}
\newcommand{\K}{\mathbf{K}}
\newcommand{\bL}{\mathbf{L}}
\newcommand{\M}{\mathbf{M}}
\newcommand{\bO}{\mathbf{O}}
\newcommand{\bP}{\mathbf{P}}
\newcommand{\Q}{\mathbf{Q}}
\newcommand{\R}{\mathbf{R}}
\newcommand{\bS}{\mathbf{S}}
\newcommand{\T}{\mathbf{T}}
\newcommand{\U}{\mathbf{U}}
\newcommand{\V}{\mathbf{V}}
\newcommand{\W}{\mathbf{W}}
\newcommand{\X}{\mathbf{X}}
\newcommand{\Y}{\mathbf{Y}}
\newcommand{\Z}{\mathbf{Z}}

\newcommand{\ba}{\mathbf{a}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\bc}{\mathbf{c}}
\newcommand{\bd}{\mathbf{d}}
\newcommand{\be}{\mathbf{e}}
\newcommand{\f}{\mathbf{f}}
\newcommand{\g}{\mathbf{g}}
\newcommand{\h}{\mathbf{h}}
\newcommand{\bk}{\mathbf{k}}
\newcommand{\m}{\mathbf{m}}
\newcommand{\n}{\mathbf{n}}
\newcommand{\p}{\mathbf{p}}
\newcommand{\q}{\mathbf{q}}
\newcommand{\br}{\mathbf{r}}
\newcommand{\s}{\mathbf{s}}
\newcommand{\bt}{\mathbf{t}}
\newcommand{\bu}{\mathbf{u}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\w}{\mathbf{w}}
\newcommand{\x}{\mathbf{x}}
\newcommand{\y}{\mathbf{y}}
\newcommand{\z}{\mathbf{z}}

% Symbols
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}
%\newcommand{\cPi}{\mathcal{\Pi}}

\newcommand{\bp}{\bar{\p}}
\newcommand{\BP}{\bar{\bP}}

\def\bphi{\mbox{\boldmath $\phi$}}
\def\bdelta{\mbox{\boldmath $\delta$}}
\def\blambda{\mbox{\boldmath $\lambda$}}
\def\bLambda{\mbox{\boldmath $\Lambda$}}
% \def\bSigma{\mbox{\boldmath $\Sigma$}}
\def\bPi{\mbox{\boldmath $\Pi$}}
% \def\bTheta{\mbox{\boldmath $\Theta$}}
\newcommand{\bTheta}{\mathbf{\Theta}}
\newcommand{\bSigma}{\mathbf{\Sigma}}
\newcommand{\one}{\mathbf{1}}
\newcommand{\zero}{\mathbf{0}}
\newcommand{\epi}{\mathbf{epi}}
\newcommand{\dom}{\mathbf{dom}}
\newcommand{\real}{\mathbb{R}}
\newcommand{\bina}{\{0, 1\}}
\newcommand{\integer}{\mathbb{Z}}
\newcommand{\acc}{\text{acc}}
\newcommand{\err}{\text{err}}
\newcommand{\dist}{\text{dist}}
\newcommand{\convA}{\stackbin[\A]{}{*}}
\newcommand{\convAj}{\stackbin{\A_j}{*}}
\newcommand{\Searrow}{\rotatebox[origin=c]{-45}{$\Rightarrow$}}
\newcommand{\udots}{\mathinner{\mskip1mu\raise1pt\vbox{\kern7pt\hbox{.}}\mskip2mu\raise4pt\hbox{.}\mskip2mu\raise7pt\hbox{.}\mskip1mu}}

%\def\convt{\llcorner\joinrel\mathrel*\joinrel\lrcorner}
\def\astm{\ \dot{*}_m  }
\def\astmm{\ \ddot{*}_m  }
\def\astl{\ \dot{*}_l \ }
\def\astll{\ \ddot{*}_l \ }
\def\astx{ \dot{*}_{n_x}  }
\def\astxx{ \ddot{*}_{n_x}  }
\def\asts{ \ \dot{*}_{n_s} }
\def\astss{ \ \ddot{*}_{n_s} }
\def\astsss{ \ \dddot{*}_{n_s} }
\def\astz{ \ \dot{*}_{n_z}  }
\def\astzz{ \ \ddot{*}_{n_z}  }
%\renewcommand\arraystretch{1.5}

% for DGM paper
%\newcommand{\Hl}{\overleftarrow{\bH}}
\newcommand{\Hl}{\overleftarrow{\bH}}
\newcommand{\Hr}{\overrightarrow{\bH}}
\newcommand{\dk}{\dot{k}}
\newcommand{\dd}{\dot{d}}
\newcommand{\hQ}{\hat{\Q}}

% Operations
% \DeclareMathOperator*{\argmin}{arg\,min}
% \DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\tra}{tr}
\DeclareMathOperator*{\eig}{eig}
\DeclareMathOperator*{\diag}{diag}
\DeclareMathOperator*{\Diag}{Diag}
\DeclareMathOperator*{\sgn}{sign}
\DeclareMathOperator*{\vect}{vec}
\DeclareMathOperator*{\where}{where}
\DeclareMathOperator*{\st}{s.t.}
\DeclareMathOperator*{\andd}{and}
\DeclareMathOperator*{\orr}{or}
\DeclareMathOperator*{\ifff}{if}
\DeclareMathOperator*{\const}{const}
\DeclareMathOperator*{\jvmin}{\mathnormal{J(v)}\,=\,min}

% \makeatletter
% \DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
% \def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
% \def\aka{\emph{a.k.a}\onedot} \def\Aka{\emph{A.k.a}\onedot}
% \def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
% \def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
% \def\cf{\emph{c.f}\onedot} \def\Cf{\emph{C.f}\onedot}
% \def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
% \def\wrt{w.r.t\onedot} \def\dof{d.o.f\onedot}
% % \def\etal{\emph{et al}\onedot}
% \makeatother

\newcommand\etal{\emph{et al.}}
\newcommand\eg{\emph{e.g.}}
\newcommand\ie{\emph{i.e.}}
\newcommand\wrt{\emph{w.r.t.}}
\newcommand\aka{\emph{a.k.a.}}
\newenvironment{aligns}{\par\nobreak\small\noindent\align}{\endalign}
\]
\end{document}
